Neural-based Modeling for Performance Tuning of Spark Data Analytics

Cloud data analytics has become an integral part of enterprise business operations for data-driven insight discovery. Performance modeling of cloud data analytics is crucial for performance tuning and other critical operations in the cloud. Traditional modeling techniques fail to adapt to the high degree of diversity in workloads and system behaviors in this domain. In this paper, we bring recent Deep Learning techniques to bear on the process of automated performance modeling of cloud data analytics, with a focus on Spark data analytics as representative workloads. At the core of our work is the notion of learning workload embeddings (with a set of desired properties) to represent fundamental computational characteristics of different jobs, which enable performance prediction when used together with job configurations that control resource allocation and other system knobs. Our work provides an in-depth study of different modeling choices that suit our requirements. Results of extensive experiments reveal the strengths and limitations of different modeling methods, as well as superior performance of our best performing method over a state-of-the-art modeling tool for cloud analytics.

==> __latexindent_temp.tex <==
\vspace{-0.3in}
\begin{abstract}
	Cloud data analytics has become an integral part of enterprise business operations for  data-driven 
	insight discovery. Performance modeling of cloud data analytics is  crucial for performance tuning and 
	other critical operations in the cloud. Traditional modeling techniques fail to adapt to the high degree of 
	diversity in workloads and system behaviors in this domain.  In this paper, we bring  recent Deep 
	Learning techniques to bear on the process of automated performance 
	modeling of cloud data analytics, \RV{with a focus on Spark data analytics as representative  workloads}. 
	At the core of our work is the notion of learning workload embeddings 
	(with a set of desired properties) to represent fundamental computational characteristics of different jobs,  
	which enable  performance prediction when used together with job configurations that control 
	resource allocation and  other system knobs. 
	Our work provides  an in-depth study of different modeling choices that suit our requirements. 
	Results of  extensive experiments reveal %valuable insights including 
	the strengths and limitations 
	of different modeling methods, as well as  superior performance of our best performing method  
	over a state-of-the-art modeling tool for cloud analytics.
	
	%\keywords{First keyword  \and Second keyword \and Another keyword.}
\end{abstract}
\vspace{-0.3in}

\mysection{Introduction}

Big data analytics has become an integral part of enterprise businesses  for obtaining insights 
from  voluminous  data being generated every day. Big data analytics tasks %\RV{such as Spark-based tasks}, 
often run in the public cloud or  on  the enterprise's  private cloud. A  recent  survey reports that  currently, 65\% 
of North American enterprises rely on public cloud  platforms, and 66\% run  internal private 
clouds~\cite{forrester2020}.

Performance modeling of execution runs  (called jobs) of analytic tasks  on a cloud platform has become  
a critical  technical issue. From an analytical user's perspective, it is important to keep the {\em latency} 
of analytic jobs low in order to obtain timely insight from data, while at the same time, choose appropriate 
configurations (the number of cores, memory size, etc.) to reduce  {\em cloud  costs}, known to be a major 
part of operational expenses of companies today. From a cloud service provider's perspective, it needs to 
support  serverless computing (e.g., \cite{Aurora-serverless})  by estimating the latency of a  user 
job and deciding how  many resources to allocate  to offer the user a  cost-performance  sweet spot, 
as well as to use latency estimates to govern dispatching and admissions control~\cite{ChiMHT11}. 
Therefore, at the heart of massive-scale cloud analytics lies a critical technical issue: {\em estimate a performance  
objective (e.g., latency) of each analytic  job under a specific configuration (of resource allocation and other system 
knobs) on a cloud platform}, referred   to as the performance modeling problem in this paper. 
Then  the model can be used to tune  the  configuration in order to meet  cost-performance goals.

Performance modeling of cloud data analytics is a hard problem for several reasons: 
 First, there is a wide  spectrum of analytics tasks, such as SQL queries, user defined functions (UDFs), 
 machine learning (ML) tasks, that have different computational characteristics. Second,  analytics jobs are 
 run in a distributed  environment, involving highly complex, dynamic CPU, IO, memory, network  
 behaviors. Third, there are also many resource choices that affect performance (e.g., over 190 
  combinations of resource options covering the number of compute cores, memory, etc. 
  in  Amazon's EC2 offerings~\cite{EC2}). 

 For all of these reasons, existing modeling methods~\cite{LiDS15,RajanKCK16,Venkataraman:2016:EEP}  
 that employ manually-crafted models often fail to adapt to new analytic  workloads and resource options.
 

In this work, we bring large-scale machine learning to bear on the process of automated performance 
 modeling of cloud data analytics, \RV{with Spark analytics chosen as representative workloads that are 
 diverse in nature and widely deployed in the cloud}. 
 In this context, we explore the power of representation learning  of 
 Deep Neural Networks  (DNNs) to develop a {\em unified} solution to performance modeling, namely, 
 learning performance models of  analytic jobs solely from their runtime observations, irrespective of the 
 underlying task being SQL,  machine learning,  a mix of both, etc. At the core of our solution is the notion 
 of learning workload embeddings   for different jobs, 
 capturing their fundamental computational characteristics. Such embeddings,  
 when combined with a specific  configuration (of resources and other system knobs), 
 can be used to predict the performance of an analytic job on a cloud platform. 
  This modeling task, however,  
 is nontrivial   even for  DNNs due to complex real-world constraints in this problem domain, such as 
  the entanglement of different factors that affect performance and a limited number of observations 
  of an analytic task in training data (discussed in more detail in \S\ref{sec:system}.)
  Therefore, our work provides  an in-depth study of the different modeling choices 
  to suit the constraints of the problem domain, and reports on their effectiveness 
  for predicting latency of  both streaming and batch workloads  on top of Apache Spark~\cite{Spark} as 
  an example  distributed system.

More specifically, our contributions include the following:   



\begin{itemize}
[nosep,leftmargin=1em,labelwidth=*,align=left]
\item 
We summarize complex constraints in real-world  cloud analytics applications and 
 outline our corresponding system design  (\S\ref{sec:system}).

\item 
We formulate the performance modeling problem, with an emphasis on learning workload embeddings 
to enable performance prediction. In addition, we leverage domain knowledge to propose three 
desired properties of such workload embeddings: \textit{reconstruction}, \textit{independence},
and \textit{invariance} to job configurations. Guided by these properties, 
we explore several families of modeling choices to learn both the workload embeddings and 
prediction models for complex analytic jobs. These choices include 
 ($i$) the embedding architecture; ($ii$) deep autoencoders augmented with customized 
 disentanglement;  ($iiv$) Siamese neural networks; ($v$) hybrid architectures (\S\ref{sec:modeling}).


\item
To enable large-scale evaluation, we collected runtime traces from an extension of a  
stream analytics benchmark \cite{LiDS15} as well as  the TPCx-BB benchmark~\cite{tpcxbb}, both of which 
 involve a mix of SQL queries and ML tasks. 
Results of extensive experiments show valuable insights, including the strengths and limitations 
of different modeling methods and superior performance of our best technique over a state of the 
art modeling method for data analytics~\cite{ottertune}. Most notably, 
Siamese networks, by offering the best approximation of the invariance property of embeddings,
enable the most accurate models to be learned. 


\item End-to-end results with the best modeling technique, siamese networks, reveal reduction in runtime latency of $52.4\%$ on the streaming benchmark and $52.44\%$ on the TPCx-BB benchmark~\cite{tpcxbb}.


\end{itemize}

